IAdet: Simplest human-in-the-loop object detection

This work proposes a strategy for training models while annotating data named Intelligent Annotation (IA). IA involves three modules: (1) assisted data annotation, (2) background model training, and (3) active selection of the next datapoints. Under this framework, we open-source the IAdet tool, which is specific for single-class object detection. Additionally, we devise a method for automatically evaluating such a human-in-the-loop system. For the PASCAL VOC dataset, the IAdet tool reduces the database annotation time by $25\%$ while providing a trained model for free. These results are obtained for a deliberately very simple IAdet design. As a consequence, IAdet is susceptible to multiple easy improvements, paving the way for powerful human-in-the-loop object detection systems.

==> math.tex <==
Variables:
\begin{itemize}
   \item $r$ annotation speed in interactions per second
   \item $v$ training speed, batches per second
   \item $b$ batch size
   \item $p$ prediction time per image (in fact this should be multiplied by the number of images to compute the prediction of)
   \item $N_e = \max_{E(k)=e} k$ is the number of annotated images during epoch $e$. \item $f_E: E \to \mathbb{R} = f_N((N_1=1, \dots, N_e)) \approx \rho(f_E(e-1), N_e-N_{e-1})$ where $f$ is the model performance and $\rho$ the performance increase function.
   \item $T_K(x)$ and $T_E(x)$ are the times it takes to annotate image number $x$ or the time when we start training epoch $x$, respectively.  
\end{itemize}

The $k$th annotation starts at time:
\begin{equation}
    S_{T_K}(k) = \sum_{i=1}^{k-1} T_K(i), \quad 1 \leq k
\end{equation}

The $e$th epoch starts at time:
\begin{equation}
    S_{T_E}(e) = T_K(1)+(e-1) p + \sum_{i=1}^{e-1} \frac {N_i}  {b}\frac 1 v, \quad 1 \leq e
\end{equation}

Annotation $k$ starts at epoch:
\begin{equation}
    E(k)=\max_{S_{T_E}(e)\leq S_{T_K}(k)}e
\end{equation}

Interactions required for image $2\leq k$ and performance $f$:
\begin{equation}
    I_k(f(E(k))) = \min{(FP + 2 FN, 1+ 2(TP+FN))}
\end{equation}
where $f(E(k))$ gives the TPR, FPR, and FNR, and $I_1=2 FN$.

Annotation time $T_K(k)$ is:
\begin{equation}
    T_K(k) = \frac{I_k } { r(S_{T_K}(k))}
\end{equation}


